Motion Planning around Obstacles with Convex Optimization

Trajectory optimization offers mature tools for motion planning in high-dimensional spaces under dynamic constraints. However, when facing complex configuration spaces, cluttered with obstacles, roboticists typically fall back to sampling-based planners that struggle in very high dimensions and with continuous differential constraints. Indeed, obstacles are the source of many textbook examples of problematic nonconvexities in the trajectory-optimization problem. Here we show that convex optimization can, in fact, be used to reliably plan trajectories around obstacles. Specifically, we consider planning problems with collision-avoidance constraints, as well as cost penalties and hard constraints on the shape, the duration, and the velocity of the trajectory. Combining the properties of B\'ezier curves with a recently-proposed framework for finding shortest paths in Graphs of Convex Sets (GCS), we formulate the planning problem as a compact mixed-integer optimization. In stark contrast with existing mixed-integer planners, the convex relaxation of our programs is very tight, and a cheap rounding of its solution is typically sufficient to design globally-optimal trajectories. This reduces the mixed-integer program back to a simple convex optimization, and automatically provides optimality bounds for the planned trajectories. We name the proposed planner GCS, after its underlying optimization framework. We demonstrate GCS in simulation on a variety of robotic platforms, including a quadrotor flying through buildings and a dual-arm manipulator (with fourteen degrees of freedom) moving in a confined space. Using numerical experiments on a seven-degree-of-freedom manipulator, we show that GCS can outperform widely-used sampling-based planners by finding higher-quality trajectories in less time.

==> sections/background_and_main_tools.tex <==
In this section we describe the problem of finding a shortest path in a graph of convex sets~\cite{marcucci2021shortest} and we review the main properties of B\'{e}zier curves.
The former is the optimization framework that underlies GCS,  the latter will be our choice for the parameterization of collision-free trajectories.

\subsection{Shortest Paths in Graphs of Convex Sets}
\label{sec:shortest_paths_in_gcs}
\input{sections/shortest_paths_in_gcs}

%\subsection{B\'{e}zier Curves}
%\label{sec:bezier_curves}
%\input{sections/bezier_curves}
